Segmenting Subtitles for Correcting ASR Segmentation Errors

Typical ASR systems segment the input audio into utterances using purely acoustic information, which may not resemble the sentence-like units that are expected by conventional machine translation (MT) systems for Spoken Language Translation. In this work, we propose a model for correcting the acoustic segmentation of ASR models for low-resource languages to improve performance on downstream tasks. We propose the use of subtitles as a proxy dataset for correcting ASR acoustic segmentation, creating synthetic acoustic utterances by modeling common error modes. We train a neural tagging model for correcting ASR acoustic segmentation and show that it improves downstream performance on MT and audio-document cross-language information retrieval (CLIR).

==> EACL 2020 Audio Segmentation_arXiv/ablation.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ lccc}
\toprule
\multirow{2}{*}{Model} & EDI & UMD & UMD \\
  & NMT & NMT & SMT \\
\midrule
Acous. & 20.48 & 20.39 & 21.24\\
Lex. & 23.96 & 24.97 & \textbf{21.58} \\
Lex. + Under & 24.27 & 25.84 & 21.48 \\
Lex. + Over & 24.69 & 25.88 & 21.23 \\
Full &  \textbf{24.73} & \textbf{25.92} & 21.23 \\

\bottomrule
\end{tabular}
\caption {Document-level BLEU score for the models in ablation studies. We provide the acoustic model (Acous.) and our proposed model (Full). }
\label{ablbleu}
\end{table}


==> EACL 2020 Audio Segmentation_arXiv/aqwv_ANALYSIS.tex <==
\begin{table*}[h]
\label{mqwvltopus}
\centering
\begin{tabular}{ llccc|ccc|ccc }
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & \multicolumn{3}{c}{EDI-NMT} & \multicolumn{3}{c}{UMD-NMT}  & \multicolumn{3}{c}{UMD-SMT} \\
 & & NB & TB & CS & NB & TB & CS & NB & TB & CS\\
\midrule
\multirow{3}{*}{BG} & Acous. & 0.244 & 0.288 & 0.173 & 0.337 & 0.153 & 0.105 & 0.422 & 0.173 & 0.239 \\
& Seg + Sub & \textbf{0.379} & \textbf{0.312} & \textbf{0.195} & \textbf{0.391} & \textbf{0.247} & \textbf{0.271} & 0.422 & \textbf{0.174} & 0.239 \\
& Ref & 0.366 & 0.328 & 0.244 & 0.465 & 0.212 & 0.380 & 0.448 & 0.153 & 0.414 \\
\midrule
\multirow{3}{*}{FA} & Acous.  & \textbf{0.122} & 0.058 & 0 & 0 & 0.034 & 0 & 0 & 0.009 & 0 \\
& Seg + Sub & 0.112 & \textbf{0.100} & 0 & 0 & \textbf{0.055} & 0 & 0 & 0.009 & 0 \\
& Ref &  0.470 & 0 & 0.089 & 0.009 & 0.167 & 0 & 0 & 0.170 & 0\\
\midrule
\multirow{3}{*}{LT} & Acous.  & 0.247 & \textbf{0.220} &	0.040 &	0.020 & 0.011 & \textbf{0.268} & 0.365 & \textbf{0.210} & 0.024 \\
& Seg + Sub & \textbf{0.280} & 0.209 & \textbf{0.046} & \textbf{0.093} & \textbf{0.021} & 0 & 0\textbf{.367} & 0.208 & 0.024 \\
& Ref & 0.371 & 0.302 & 0.231 & 0.050 & 0.064 & 0.142 & 0.463 & 0.228 & 0.247 \\

\bottomrule
\end{tabular}
\caption {AQWV scores on ANALYSIS set.}
\label{aqwvanalysis}
\end{table*}

==> EACL 2020 Audio Segmentation_arXiv/aqwv_ANALYSIS_new.tex <==
\begin{table}[t]
\label{mqwvltopus}
\centering
\begin{tabular}{ ll ccc}
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & EDI & UMD & UMD \\
  & & NMT & NMT & SMT \\
\midrule
\multirow{3}{*}{BG} & Acous. & 0.307 & 0.240 & 0.304 \\
& Seg + Sub & 0.\textbf{332} & \textbf{0.331} & 0.304 \\
& Ref & 0.356 & 0.358 & 0.335 \\
\midrule
\multirow{3}{*}{FA} & Acous.  & 0.057 & 0.018 & 0.012 \\
& Seg + Sub & \textbf{0.063} & 0.018 & 0.012 \\
& Ref &  0.259 &0.089 & 0.059 \\
\midrule
\multirow{3}{*}{LT} & Acous. & 0.243 & 0.112 & 0.290 \\
& Seg + Sub & \textbf{0.253} & 0.071 & 0.290 \\
& Ref & 0.361 & 0.093 & 0.370 \\
\bottomrule
\end{tabular}
\caption {AQWV scores on ANALYSIS set.}
\label{aqwvanalysis}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/aqwv_DEV.tex <==
\begin{table*}[h]
\label{mqwvltopus}
\centering
\begin{tabular}{ llccc|ccc|ccc }
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & \multicolumn{3}{c}{EDI-NMT} & \multicolumn{3}{c}{UMD-NMT}  & \multicolumn{2}{c}{UMD-SMT} \\
 & & NB & TB & CS & NB & TB & CS & NB & TB & CS\\
\midrule
\multirow{2}{*}{BG} & Acous. & 0.437 & 0.168 & 0.086 & 0.544 & 0.187 & 0.225 & 0.570 & 0.119 & 0.117 \\
& Seg + Sub & \textbf{0.520} & \textbf{0.219} & \textbf{0.122} & \textbf{0.551} & \textbf{0.194} & \textbf{0.230} & 0.570 & \textbf{0.121} & 0.117 \\
\midrule
\multirow{2}{*}{FA} & Acous.  & \\
& Seg + Sub & \\
\midrule
\multirow{2}{*}{LT} & Acous.  & 0.091 & 0.140 & 0.269 & 0.050 & 0.064 & 0.146 & 0.246 & 0.283 & 0.267 \\
& Seg + Sub & \textbf{0.196} & \textbf{0.173} & \textbf{0.273} & \textbf{0.153} & \textbf{0.084} & 0.117 & \textbf{0.248} & 0.283 & 0.267 \\
\bottomrule
\end{tabular}
\caption {AQWV scores on DEV set.}
\label{aqwvdev}
\end{table*}

==> EACL 2020 Audio Segmentation_arXiv/aqwv_DEV_new.tex <==
\begin{table}[t]
\label{mqwvltopus}
\centering
\begin{tabular}{ ll ccc }
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & EDI & UMD  & UMD \\
  & & NMT & NMT & SMT \\
\midrule
\multirow{2}{*}{BG} & Acous. & 0.241 & 0.328 & 0.266 \\
& Seg + Sub & \textbf{0.291} & 0.328 & 0.266 \\
\midrule
\multirow{2}{*}{FA} & Acous.  & 0.031 & 0 & 0.020\\
& Seg + Sub & 0.032 & 0 & 0.020\\
\midrule
\multirow{2}{*}{LT} & Acous. & 0.191 & 0.092 & 0.328\\
& Seg + Sub & \textbf{0.204} & \textbf{0.153} & 0.328 \\
\bottomrule
\end{tabular}
\caption {AQWV scores on DEV set.}
\label{aqwvdev}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/aqwv_EVAL.tex <==
\begin{table}[ht]
\label{mqwvltopus}
\centering
\begin{tabular}{ llccc}
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & EDI & UMD & UMD \\
     & & NMT & NTM & SMT \\
\midrule
\multirow{2}{*}{LT} & Acous. & 0.292 & 0.175 & 0.328 \\
& Seg + Sub & \textbf{0.293} & \textbf{0.179} & \textbf{0.399} \\
\bottomrule
\end{tabular}
\caption {MQWV scores on the Test (Large) set.}
\label{aqwveval}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/aqwv_ablation.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ l ccc}
\toprule
 Model & EDI & UMD & SMT \\
\midrule
Acous. & 0.307 & 0.240 & 0.304 \\
Sub (No Segment) & 0.342 & 0.305 & 0.328 \\
Sub (Under-seg.) & 0.332 & 0.328 & 0. \\
Sub (Over-seg.) & \textbf{0.356} & 0.331 & 0.\\
Sub &  0.332 & \textbf{0.358} & 0.335 \\

\bottomrule
\end{tabular}
\caption {AQWV scores on ablation studies.}
\label{aqwvablation}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/aqwv_comb.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ ll ccc}
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & EDI & UMD & UMD \\
  & & NMT & NMT & SMT \\
\midrule
\multirow{3}{*}{BG} & Acous. & 0.173 & 0.134 & 0.164  \\
& Seg + Sub &  \textbf{0.177} & \textbf{0.180} & 0.164 \\
\midrule
\multirow{3}{*}{FA} & Acous. & 0.040 & 0.039 &  0.046 \\
& Seg + Sub & \textbf{0.071} & \textbf{0.042} & \textbf{0.145} \\
\midrule
\multirow{3}{*}{LT} & Acous. & 0.128 & \textbf{0.067} & 0.157 \\
& Seg + Sub &  \textbf{0.136} & 0.060 & \textbf{0.172} \\
\bottomrule
\end{tabular}
\caption {MQWV scores on Test (Small) set.}
\label{mqwvopus}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/bleu_ANALYSIS.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ llccc}
\toprule
\multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & EDI & UMD  & UMD \\
& & NMT & NMT & SMT\\
\midrule
\multirow{4}{*}{BG} & Acous. & 20.48\phantom{*} & 20.39\phantom{*} & \textbf{21.24} \\
& Seg & 22.38* & 23.35* & 21.23 \\
& Seg + Sub &  \textbf{24.73*} & \textbf{25.92*} & 21.23 \\
\cmidrule(lr){2-5}
& Align & 24.98\phantom{*} & 27.81\phantom{*} & 21.29 \\
& Ref & 43.75\phantom{*} & 35.40\phantom{*} & 29.50 \\
\midrule
\multirow{3}{*}{FA} & Acous. & 5.35\phantom{*} & 6.26\phantom{*} & \textbf{4.54} \\
& Seg & 5.32\phantom{*} & 6.22\phantom{*} & 3.28 \\ 
& Seg + Sub &  \textbf{6.47*} & \textbf{6.83*} & 4.50 \\
\cmidrule(lr){2-5}
& Align &  7.67\phantom{*} & 7.02\phantom{*} & 4.59 \\
& Ref & 17.08\phantom{*} & 11.24\phantom{*} & 7.76 \\
\midrule
\multirow{4}{*}{LT} & Acous. & 15.20\phantom{*} & \textbf{8.38}\phantom{*} & 14.76 \\
& Seg & 15.18\phantom{*} & 8.34\phantom{*} & 14.76 \\
& Seg + Sub & \textbf{15.22}\phantom{*} & 8.33\phantom{*} & 14.76 \\
\cmidrule(lr){2-5}
& Align & 15.60\phantom{*} & 8.71\phantom{*} & 14.84 \\
& Ref &  20.40\phantom{*} & 11.94\phantom{*} & 21.30  \\
\bottomrule
\end{tabular}
\caption {Document-level BLEU scores on ANALYSIS set. * represents statistical significance when compared to Acous. at the 0.05 level.
We show the result of translations using the original acoustic segmentation (Acous.), our model trained only on the BUILD dataset (Seg), and our full model (Seg + Sub). For reference, we provide the scores of translation on ASR tokens aligned to the reference transcription segmentation (Align), and the reference transcription (Ref). }
\label{bleu}
\end{table}


==> EACL 2020 Audio Segmentation_arXiv/bleu_quartiles.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ ll ccc}
\toprule
 ARI & \multirow{2}{*}{Model} & EDI & UMD \\
  Quartile & & NMT & NMT \\
\midrule
\multirow{2}{*}{Q1} & Acous. & 17.78 & \textbf{24.70} \\
& Seg + Sub & \textbf{17.92} & 11.62 \\
\midrule
\multirow{2}{*}{Q2} & Acous.  & 20.76 & 22.09 \\
& Seg + Sub & \textbf{26.89} & \textbf{31.24} \\
\midrule
\multirow{2}{*}{Q3} & Acous. & 22.87 & 20.38 \\
& Seg + Sub & \textbf{29.96} & \textbf{33.22} \\
\midrule
\multirow{2}{*}{Q4} & Acous.  & 23.41 & 21.00 \\
& Seg + Sub & \textbf{29.87} & \textbf{35.24} \\
\bottomrule
\end{tabular}
\caption {Bulgarian BLEU scores on Test (Small) (transcribed portion) when separated into quartiles by sentence complexity (as measured by ARI).}
\label{tab:bleu_quartiles}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/bleu_quartiles_bg_full.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{ ll ccc}
\toprule
 ARI & \multirow{2}{*}{Model} & EDI & UMD & UMD \\
  Quartile & & NMT & NMT & SMT \\
\midrule
\multirow{2}{*}{Q1} & Acous. & 17.78 & \textbf{24.70} & 22.26 \\
& Seg + Sub & \textbf{17.92} & 11.62 & \textbf{22.58} \\
\midrule
\multirow{2}{*}{Q2} & Acous.  & 20.76 & 22.09 & 23.35 \\
& Seg + Sub & \textbf{26.89} & \textbf{31.24} & \textbf{23.43} \\
\midrule
\multirow{2}{*}{Q3} & Acous. & 22.87 & 20.38 & \textbf{22.45} \\
& Seg + Sub & \textbf{29.96} & \textbf{33.22} & 21.68 \\
\midrule
\multirow{2}{*}{Q4} & Acous.  & 23.41 & 21.00 & 22.97 \\
& Seg + Sub & \textbf{29.87} & \textbf{35.24} & \textbf{23.25} \\
\bottomrule
\end{tabular}
\caption {Bulgarian BLEU scores on Test (Small) (transcribed portion) when separated into quartiles by sentence complexity (as measured by ARI).}
\label{tab:bleu_quartiles_bg_full}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/bleu_quartiles_fa_full.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{ ll ccc}
\toprule
 ARI & \multirow{2}{*}{Model} & EDI & UMD & UMD \\
  Quartile & & NMT & NMT & SMT \\
\midrule
\multirow{2}{*}{Q1} & Acous.  & 3.46 & 3.40 & 3.21 \\
& Seg + Sub & \textbf{6.05} & \textbf{4.49} & \textbf{3.43} \\
\midrule
\multirow{2}{*}{Q2} & Acous. & 3.55 & 3.87 & 3.22 \\
& Seg + Sub & \textbf{5.06} & \textbf{5.41} & \textbf{3.66} \\
\midrule
\multirow{2}{*}{Q3} & Acous. & 4.71 & 5.33 & 5.19 \\
& Seg + Sub & \textbf{7.44} & \textbf{7.29} & \textbf{5.54} \\
\midrule
\multirow{2}{*}{Q4} & Acous.  & 5.88 & 6.15 & 3.90 \\
& Seg + Sub & \textbf{7.81} & \textbf{7.59} & \textbf{4.47} \\
\bottomrule
\end{tabular}
\caption {Farsi BLEU scores on Test (Small) (transcribed portion) when separated into quartiles by sentence complexity (as measured by ARI).}
\label{tab:bleu_quartiles_fa_full}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/bleu_quartiles_lt_full.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{ ll ccc}
\toprule
 ARI & \multirow{2}{*}{Model} & EDI & UMD & UMD \\
  Quartile & & NMT & NMT & SMT \\
\midrule
\multirow{2}{*}{Q1} & Acous. & 4.24 & \textbf{3.13} & \textbf{5.14} \\
& Seg + Sub & \textbf{4.32} & 2.76 & 5.11 \\
\midrule
\multirow{2}{*}{Q2} & Acous.  & \textbf{14.07} & \textbf{7.18} & \textbf{13.45} \\
& Seg + Sub & 14.01 & 6.83 & 13.39 \\
\midrule
\multirow{2}{*}{Q3} & Acous. & 15.95 & 7.81 & 14.85 \\
& Seg + Sub & \textbf{16.39} & \textbf{8.13} & \textbf{14.87} \\
\midrule
\multirow{2}{*}{Q4} & Acous.  & \textbf{15.41} & \textbf{7.94} & 15.85 \\
& Seg + Sub & 14.60 & 7.78 & \textbf{15.87} \\
\bottomrule
\end{tabular}
\caption {Lithuanian BLEU scores on Test (Small) (transcribed portion) when separated into quartiles by sentence complexity (as measured by ARI).}
\label{tab:bleu_quartiles_lt_full}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/dataset.tex <==

\begin{table*}
\centering
\begin{tabular}{c ccc ccc  ccc ccc  ccc }
\toprule
 \multirow{2}{*}{Lang.} & \multicolumn{3}{c}{OpenSubtitles} & \multicolumn{3}{c}{\BUILD~Train} & \multicolumn{3}{c}{\BUILD~Valid}  \\
 \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
 & D & I & S & D & I & S & D & I & S  \\
 \midrule
BG & 2000 & \phantom{0,}459,301 & \phantom{0}3.95 & 352 & \phantom{0}7,723 & 3.22 & 108 & 2,472 & 3.14    \\
FA & 2000 & \phantom{0,}120,039 & \phantom{0}3.88 & 302 & \phantom{0}6,707 & 3.52 & 120 & 2,679 & 3.53  \\
LT & 1977 & \phantom{0,}165,751 & 12.99 & 484 & 11,782 & 3.40 & 112 & 2,893 & 3.31  \\
\bottomrule
\end{tabular}
\caption{Segmentation model training dataset statistics. We report number of documents (D), number of instances (I) in each dataset and average number of segments
per instance (S).}
\label{tab:dataset}
\end{table*}



\begin{table}
\centering
\begin{tabular}{c cccc  }
\toprule
 Lang. & \multicolumn{2}{c}{Test (Small)} & \multicolumn{2}{c}{Test (Large)} \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5}
 &Q & D & Q &D\\
 \midrule
BG & 300  & 634 & -- & --\\
FA & 221  & 528 & -- & -- \\
LT & 300  & 496 & 1,000   & 3,297 \\
\bottomrule
\end{tabular}
\caption{Number of queries (Q) and documents (D) in the speech retrieval test collections. } %

\label{tab:testdataset}
\end{table}

==> EACL 2020 Audio Segmentation_arXiv/human_eval.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{ c c cc | cc }
\toprule
\multirow{2}{*}{Lang.} & \multirow{2}{*}{MT} &  \multicolumn{2}{c}{Relevance} & \multicolumn{2}{c}{Quality}  \\
&   & A & M & A & M \\
  \midrule
  \multirow{4}{*}{BG} 
 & EDI-NMT &   0.682 & 0.798** & 0.463 & 0.74* \\
 & UMD-NMT &  0.763 & 0.753 & 0.387 & 0.34 \\
   & UMD-SMT & 0.7 &  0.837** & 0.333 & 0.584*\\
  & Reference & \multicolumn{2}{c}{0.916} & \multicolumn{2}{c}{1.32} \\
   \midrule
\bottomrule
\end{tabular}
\caption {Passage-level evaluation comparing relevance using the Sub model (M), the acoustic baseline (A).Evaluation of reference translation is also provided for each language. p$<$0.1*, p$<$0.05** }
\label{tab:human}

\end{table*}

==> EACL 2020 Audio Segmentation_arXiv/macros.tex <==
\newcommand{\tokens}{\mathbf{x}}
\newcommand{\token}{x}
\newcommand{\ctags}{\mathbf{y}}
\newcommand{\ctag}{y}
\newcommand{\numToks}{n}
\newcommand{\atags}{\boldsymbol{\gamma}}
\newcommand{\atag}{\gamma}
\newcommand{\tokVocab}{\mathcal{V}}
\newcommand{\reals}[1]{\mathbb{R}^{#1}}
\newcommand{\binspace}[1]{\{0,1\}^{#1}}
\newcommand{\model}{p}
\newcommand{\params}{\theta}
\newcommand{\usegprob}{\check{\alpha}}
\newcommand{\utags}{\boldsymbol{\check{\atags}}}
\newcommand{\otags}{\boldsymbol{\hat{\atags}}}
\newcommand{\osegprob}{\hat{\alpha}}
\newcommand{\bernoulli}[1]{\operatorname{Bernoulli}(#1)}
\newcommand{\numSegs}{m}
\newcommand{\joinprob}{\kappa}
\newcommand{\emb}{\mathbf{e}}
\newcommand{\hid}{\mathbf{h}}
\newcommand{\corpus}{\mathcal{D}}
\newcommand{\lstm}{\operatorname{LSTM}}
\newcommand{\flstm}{\overrightarrow{\lstm}}
\newcommand{\blstm}{\overleftarrow{\lstm}}

==> EACL 2020 Audio Segmentation_arXiv/newexample.tex <==
\begin{figure*}[t]
\center
\noindent\fbox{%
\resizebox{0.84\textwidth}{!}{\parbox{\textwidth}{%
    \textbf{Acoustic Segmentation (Over-segmentation):}

\begin{center}    
  ARE YOU OKAY $\blacksquare$ AGENT  SCULLY $\blacksquare$ YOU KIND OF
            SOUNDED  A  $\blacksquare$  LITTLE  SPOOKY $\blacksquare$\\
   \end{center}       
   
   \textbf{Corrected Sentence Segmentation:}
   
   \begin{center}    
 ARE YOU OKAY AGENT  SCULLY $\blacksquare$ YOU KIND OF
            SOUNDED  A  LITTLE  SPOOKY $\blacksquare$ \\~\\
   \end{center}  
   
   \textbf{Acoustic Segmentation (Under-segmentation):}
   \begin{center}
        NO IS HE IN SOME KIND OF TROUBLE $\blacksquare$
   \end{center}
   
      \textbf{Corrected Sentence Segmentation:}

\begin{center}
         NO $\blacksquare$ IS HE IN SOME KIND OF TROUBLE $\blacksquare$
   \end{center}
   
   

   
    }}}
    \caption{Example acoustic segmentation errors and their corrections. $\blacksquare$ indicates a segment boundary. }
    \label{fig:newexample}
\end{figure*}

==> EACL 2020 Audio Segmentation_arXiv/prev_label.tex <==
\begin{figure*}
    \centering

    \noindent\fbox{%
    \parbox{\textwidth}{%
        Yeah. The holiday market is too busy. Yes.
    \small  \center
    $\begin{array}{cccccccccccccccccc}
    & token & = & yeah & the & holiday & market & is & too & busy & yes   \\
    & label_{correct} & = & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 1  \\
    \midrule
    & label_{under} & = & 1 & - & - & - & - & - & \textbf{0} & 1    \\
    & label_{over} & = & - & 0 & 0 & \textbf{1} & 0 & \textbf{1} & - & -   \\
    \midrule
    & label_{prev} & = & 1 & 0 & 0 & 1 & 0 & 1 & 0 & 1 \\

    
    \end{array}
    $
    }%
}
    \caption{Examples of label creation that simulate undersegmentation and oversegmentation. We show first the label simulating the two problems separately, and then the final label. }
    \label{fig:tv-example}
\end{figure*}

==> EACL 2020 Audio Segmentation_arXiv/synthexample.tex <==
\begin{figure*}[t]
    \centering

    \noindent\resizebox{\textwidth}{!}{\fbox{%
    \parbox{1.02\textwidth}{%
    \textbf{Reference Segmentation:}
    
    \begin{center}
        YEAH $\blacksquare$ THE HOLIDAY MARKET IS TOO BUSY $\blacksquare$ YES $\blacksquare$
        \end{center}
    
    
    
    \textbf{Synthetic Acoustic Segmentation Generation:} \\
    $\begin{array}{rrccccccccccccccccc}
    \toprule
    \textrm{Model Output: } & \ctags  & = & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 1  \\
    \midrule
     \textrm{(Under-seg.) } & \utags & = & 1 & - & - & - & - & - & \textbf{0} & 1    \\
     \textrm{(Over-seg.) } & \otags& = & - & 0 & 0 & \textbf{1} & 0 & \textbf{1} & - & -   \\
    \midrule
  \multirow{2}{*}{\textrm{Model Input: }}    & \atags & = & 1 & 0 & 0 & 1 & 0 & 1 & 0 & 1 \\
    & \tokens & = & YEAH & THE & HOLIDAY & MARKET & IS & TOO & BUSY & YES   \\
    \bottomrule

    
    \end{array}
    $
    
    
    
    \textbf{Synthetic Acoustic Segmentation ($\atags$):}
    
    \begin{center}
        YEAH $\blacksquare$ THE HOLIDAY MARKET $\blacksquare$ IS TOO $\blacksquare$ BUSY YES $\blacksquare$
    \end{center}
    
    }%
    }}
    \caption{Example of synthetic acoustic segmentation ($\atags$) creation. For each training datapoint, we have as model input the tokens $\tokens$ and the corresponding model output sentence boundary labels $\ctags$. To generate the synthetic acoustic segmentation ($\atags$), we apply under-segmentation ($\utags$) and over-segmentation ($\otags$) noise to $\ctags$. Dashes indicate the tokens where the particular noise is not applicable. Bold indicates the changed labels due to the noise. We generate the additional input $\atags$ by combining both $\utags$ and $\otags$.
    }
    \label{fig:synthexample}
\end{figure*}

==> aqwv_ANALYSIS.tex <==
\begin{table*}[h]
\label{mqwvltopus}
\centering
\begin{tabular}{ llccc|ccc|ccc }
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & \multicolumn{3}{c}{EDI-NMT} & \multicolumn{3}{c}{UMD-NMT}  & \multicolumn{3}{c}{UMD-SMT} \\
 & & NB & TB & CS & NB & TB & CS & NB & TB & CS\\
\midrule
\multirow{3}{*}{BG} & Acous. & 0.244 & 0.288 & 0.173 & 0.337 & 0.153 & 0.105 & 0.422 & 0.173 & 0.239 \\
& Seg + Sub & \textbf{0.379} & \textbf{0.312} & \textbf{0.195} & \textbf{0.391} & \textbf{0.247} & \textbf{0.271} & 0.422 & \textbf{0.174} & 0.239 \\
& Ref & 0.366 & 0.328 & 0.244 & 0.465 & 0.212 & 0.380 & 0.448 & 0.153 & 0.414 \\
\midrule
\multirow{3}{*}{FA} & Acous.  & \textbf{0.122} & 0.058 & 0 & 0 & 0.034 & 0 & 0 & 0.009 & 0 \\
& Seg + Sub & 0.112 & \textbf{0.100} & 0 & 0 & \textbf{0.055} & 0 & 0 & 0.009 & 0 \\
& Ref &  0.470 & 0 & 0.089 & 0.009 & 0.167 & 0 & 0 & 0.170 & 0\\
\midrule
\multirow{3}{*}{LT} & Acous.  & 0.247 & \textbf{0.220} &	0.040 &	0.020 & 0.011 & \textbf{0.268} & 0.365 & \textbf{0.210} & 0.024 \\
& Seg + Sub & \textbf{0.280} & 0.209 & \textbf{0.046} & \textbf{0.093} & \textbf{0.021} & 0 & 0\textbf{.367} & 0.208 & 0.024 \\
& Ref & 0.371 & 0.302 & 0.231 & 0.050 & 0.064 & 0.142 & 0.463 & 0.228 & 0.247 \\

\bottomrule
\end{tabular}
\caption {AQWV scores on ANALYSIS set.}
\label{aqwvanalysis}
\end{table*}

==> aqwv_ANALYSIS_new.tex <==
\begin{table}[t]
\label{mqwvltopus}
\centering
\begin{tabular}{ ll ccc}
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & EDI & UMD & UMD \\
  & & NMT & NMT & SMT \\
\midrule
\multirow{3}{*}{BG} & Acous. & 0.307 & 0.240 & 0.304 \\
& Seg + Sub & 0.\textbf{332} & \textbf{0.331} & 0.304 \\
& Ref & 0.356 & 0.358 & 0.335 \\
\midrule
\multirow{3}{*}{FA} & Acous.  & 0.057 & 0.018 & 0.012 \\
& Seg + Sub & \textbf{0.063} & 0.018 & 0.012 \\
& Ref &  0.259 &0.089 & 0.059 \\
\midrule
\multirow{3}{*}{LT} & Acous. & 0.243 & 0.112 & 0.290 \\
& Seg + Sub & \textbf{0.253} & 0.071 & 0.290 \\
& Ref & 0.361 & 0.093 & 0.370 \\
\bottomrule
\end{tabular}
\caption {AQWV scores on ANALYSIS set.}
\label{aqwvanalysis}
\end{table}

==> aqwv_DEV.tex <==
\begin{table*}[h]
\label{mqwvltopus}
\centering
\begin{tabular}{ llccc|ccc|ccc }
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & \multicolumn{3}{c}{EDI-NMT} & \multicolumn{3}{c}{UMD-NMT}  & \multicolumn{2}{c}{UMD-SMT} \\
 & & NB & TB & CS & NB & TB & CS & NB & TB & CS\\
\midrule
\multirow{2}{*}{BG} & Acous. & 0.437 & 0.168 & 0.086 & 0.544 & 0.187 & 0.225 & 0.570 & 0.119 & 0.117 \\
& Seg + Sub & \textbf{0.520} & \textbf{0.219} & \textbf{0.122} & \textbf{0.551} & \textbf{0.194} & \textbf{0.230} & 0.570 & \textbf{0.121} & 0.117 \\
\midrule
\multirow{2}{*}{FA} & Acous.  & \\
& Seg + Sub & \\
\midrule
\multirow{2}{*}{LT} & Acous.  & 0.091 & 0.140 & 0.269 & 0.050 & 0.064 & 0.146 & 0.246 & 0.283 & 0.267 \\
& Seg + Sub & \textbf{0.196} & \textbf{0.173} & \textbf{0.273} & \textbf{0.153} & \textbf{0.084} & 0.117 & \textbf{0.248} & 0.283 & 0.267 \\
\bottomrule
\end{tabular}
\caption {AQWV scores on DEV set.}
\label{aqwvdev}
\end{table*}

==> aqwv_DEV_new.tex <==
\begin{table}[t]
\label{mqwvltopus}
\centering
\begin{tabular}{ ll ccc }
\toprule
 \multirow{2}{*}{Lang.} & \multirow{2}{*}{Model} & EDI & UMD  & UMD \\
  & & NMT & NMT & SMT \\
\midrule
\multirow{2}{*}{BG} & Acous. & 0.241 & 0.328 & 0.266 \\
& Seg + Sub & \textbf{0.291} & 0.328 & 0.266 \\
\midrule
\multirow{2}{*}{FA} & Acous.  & 0.031 & 0 & 0.020\\
& Seg + Sub & 0.032 & 0 & 0.020\\
\midrule
\multirow{2}{*}{LT} & Acous. & 0.191 & 0.092 & 0.328\\
& Seg + Sub & \textbf{0.204} & \textbf{0.153} & 0.328 \\
\bottomrule
\end{tabular}
\caption {AQWV scores on DEV set.}
\label{aqwvdev}
\end{table}

==> aqwv_ablation.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ l ccc}
\toprule
 Model & EDI & UMD & SMT \\
\midrule
Acous. & 0.307 & 0.240 & 0.304 \\
Sub (No Segment) & 0.342 & 0.305 & 0.328 \\
Sub (Under-seg.) & 0.332 & 0.328 & 0. \\
Sub (Over-seg.) & \textbf{0.356} & 0.331 & 0.\\
Sub &  0.332 & \textbf{0.358} & 0.335 \\

\bottomrule
\end{tabular}
\caption {AQWV scores on ablation studies.}
\label{aqwvablation}
\end{table}

==> human_eval.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{ c c cc | cc }
\toprule
\multirow{2}{*}{Lang.} & \multirow{2}{*}{MT} &  \multicolumn{2}{c}{Relevance} & \multicolumn{2}{c}{Quality}  \\
&   & A & M & A & M \\
  \midrule
  \multirow{4}{*}{BG} 
 & EDI-NMT &   0.682 & 0.798** & 0.463 & 0.74* \\
 & UMD-NMT &  0.763 & 0.753 & 0.387 & 0.34 \\
   & UMD-SMT & 0.7 &  0.837** & 0.333 & 0.584*\\
  & Reference & \multicolumn{2}{c}{0.916} & \multicolumn{2}{c}{1.32} \\
   \midrule
\bottomrule
\end{tabular}
\caption {Passage-level evaluation comparing relevance using the Sub model (M), the acoustic baseline (A).Evaluation of reference translation is also provided for each language. p$<$0.1*, p$<$0.05** }
\label{tab:human}

\end{table*}

==> prev_label.tex <==
\begin{figure*}
    \centering

    \noindent\fbox{%
    \parbox{\textwidth}{%
        Yeah. The holiday market is too busy. Yes.
    \small  \center
    $\begin{array}{cccccccccccccccccc}
    & token & = & yeah & the & holiday & market & is & too & busy & yes   \\
    & label_{correct} & = & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 1  \\
    \midrule
    & label_{under} & = & 1 & - & - & - & - & - & \textbf{0} & 1    \\
    & label_{over} & = & - & 0 & 0 & \textbf{1} & 0 & \textbf{1} & - & -   \\
    \midrule
    & label_{prev} & = & 1 & 0 & 0 & 1 & 0 & 1 & 0 & 1 \\

    
    \end{array}
    $
    }%
}
    \caption{Examples of label creation that simulate undersegmentation and oversegmentation. We show first the label simulating the two problems separately, and then the final label. }
    \label{fig:tv-example}
\end{figure*}
